Approximating Densest Subgraph in Geometric Intersection Graphs

$ \newcommand{\cardin}[1]{\left| {#1} \right|}% \newcommand{\Graph}{\Mh{\mathsf{G}}}% \providecommand{\G}{\Graph}% \renewcommand{\G}{\Graph}% \providecommand{\GA}{\Mh{H}}% \renewcommand{\GA}{\Mh{H}}% \newcommand{\VV}{\Mh{\mathsf{V}}}% \newcommand{\VX}[1]{\VV\pth{#1}}% \providecommand{\EE}{\Mh{\mathsf{E}}}% \renewcommand{\EE}{\Mh{\mathsf{E}}}% \newcommand{\Re}{\mathbb{R}} \newcommand{\reals}{\mathbb{R}} \newcommand{\SetX}{\mathsf{X}} \newcommand{\rad}{r} \newcommand{\Mh}[1]{#1} \newcommand{\query}{q} \newcommand{\eps}{\varepsilon} \newcommand{\VorX}[1]{\mathcal{V} \pth{#1}} \newcommand{\Polygon}{\mathsf{P}} \newcommand{\IntRange}[1]{[ #1 ]} \newcommand{\Space}{\overline{\mathsf{m}}} \newcommand{\pth}[2][\!]{#1\left({#2}\right)} \newcommand{\polylog}{\mathrm{polylog}} \newcommand{\N}{\mathbb N} \newcommand{\Z}{\mathbb Z} \newcommand{\pt}{p} \newcommand{\distY}[2]{\left\| {#1} - {#2} \right\|} \newcommand{\ptq}{q} \newcommand{\pts}{s}$ For an undirected graph $\mathsf{G}=(\mathsf{V}, \mathsf{E})$, with $n$ vertices and $m$ edges, the \emph{densest subgraph} problem, is to compute a subset $S \subseteq \mathsf{V}$ which maximizes the ratio $|\mathsf{E}_S| / |S|$, where $\mathsf{E}_S \subseteq \mathsf{E}$ is the set of all edges of $\mathsf{G}$ with endpoints in $S$. The densest subgraph problem is a well studied problem in computer science. Existing exact and approximation algorithms for computing the densest subgraph require $\Omega(m)$ time. We present near-linear time (in $n$) approximation algorithms for the densest subgraph problem on \emph{implicit} geometric intersection graphs, where the vertices are explicitly given but not the edges. As a concrete example, we consider $n$ disks in the plane with arbitrary radii and present two different approximation algorithms.

==> junk/err_pdflatex <==
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023/Debian) (preloaded format=pdflatex) restricted \write18 enabled.entering extended mode

(./max_density.texLaTeX2e <2023-11-01> patch level 1L3 programming layer <2024-01-22>

(/usr/share/texlive/texmf-dist/tex/latex/base/article.clsDocument Class: article 2023/05/17 v1.4n Standard LaTeX document class

(/usr/share/texlive/texmf-dist/tex/latex/base/size12.clo))\bibdata{max_density}

(./max_density.bbl

./max_density.bbl:16: LaTeX Error: Missing 'biblatex' package.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.16   {}         ) (/usr/share/texlive/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)

(junk/max_density.aux)./max_density.tex:27: Undefined control sequence.

<argument> ...enue; Urbana, IL, 61801, USA; \href                                                   {mailto:spam@illinois.edu}...l.27 \maketitle               ./max_density.tex:27: Undefined control sequence.

<argument> ...ois.edu}{sariel@illinois.edu}; \url                                                   {http://sarielhp.org/}.l.27 \maketitle               ./max_density.tex:27: Undefined control sequence.

<argument> ...n Institute of Science (IISc); \url                                                   {saladi@iisc.ac.in}. l.27 \maketitle               ./max_density.tex:48: Undefined control sequence.l.48 ...sf{G}=(\mathsf{V},\mathsf{E})$, the \emphi                                                  {density} of a set./max_density.tex:50: Undefined control sequence.l.50 ...n $\mathsf{E}_S \subseteq \mathsf{E}\mleft                                                  ({\mathsf{G}}\mright)$ has...

./max_density.tex:50: Undefined control sequence.l.50 ...seteq \mathsf{E}\mleft({\mathsf{G}}\mright                                                  )$ has both its vertices i...

./max_density.tex:51: Undefined control sequence.l.51 the \emphw               {densest subgraph problem}, the goal is to find a subset of


LaTeX Warning: Citation `cs-dseac-12' on page 1 undefined on input line 54.




LaTeX Warning: Citation `gkt-dldsm-05' on page 1 undefined on input line 55.




LaTeX Warning: Citation `chkz-rdq2l-03' on page 1 undefined on input line 56.




LaTeX Warning: Citation `bkv-dssm-12' on page 1 undefined on input line 56.




LaTeX Warning: Citation `lmfb-sdsp-23' on page 1 undefined on input line 58.

[1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.map}{/usr/share/texmf/fonts/enc/dvips/cm-super/cm-super-ts1.enc}]./max_density.tex:64: Undefined control sequence.l.64 \NPHard            ), the densest subgraph can be computed (exactly) in polynomial


LaTeX Warning: Citation `g-fmds-84' on page 2 undefined on input line 65.

./max_density.tex:66: Undefined control sequence.

<recently read> \xspace                         l.66 ...-cut problem. Gallo \textit{et~al.}\xspace                                                  


LaTeX Warning: Citation `ggt-fpmfa-89' on page 2 undefined on input line 67.




LaTeX Warning: Citation `c-gaafd-00' on page 2 undefined on input line 68.




LaTeX Warning: Citation `ks-fds-09' on page 2 undefined on input line 70.




LaTeX Warning: Citation `c-gaafd-00' on page 2 undefined on input line 75.

./max_density.tex:78: Undefined control sequence.

<recently read> \xspace                         l.78 ...After that, Bahmani \textit{et~al.}\xspace                                                  


LaTeX Warning: Citation `bgm-epgam-14' on page 2 undefined on input line 79.

./max_density.tex:81: Undefined control sequence.l.81 $O\mleft             ({ (m/\varepsilon^2)\log n}\mright)$ time.  The problem was als...

./max_density.tex:81: Undefined control sequence.l.81 $O\mleft({ (m/\varepsilon^2)\log n}\mright                                               )$ time.  The problem was als...

./max_density.tex:83: Undefined control sequence.

<recently read> \xspace                         l.83 McGregor \textit{et~al.}\xspace                                     \cite{mtvv-dsdgs-15} and Esfandiari \te...




LaTeX Warning: Citation `mtvv-dsdgs-15' on page 2 undefined on input line 83.

./max_density.tex:83: Undefined control sequence.

<recently read> \xspace                         l.83 ...-15} and Esfandiari \textit{et~al.}\xspace                                                  


LaTeX Warning: Citation `ehw-baaus-16' on page 2 undefined on input line 84.




LaTeX Warning: Citation `bhnt-stamd-15' on page 2 undefined on input line 88.




LaTeX Warning: Citation `sw-nfdds-20' on page 2 undefined on input line 88.




LaTeX Warning: Citation `els-edsc-15' on page 2 undefined on input line 88.




LaTeX Warning: Citation `ap-naghs-14' on page 2 undefined on input line 101.




LaTeX Warning: Citation `chq-flbag-20' on page 2 undefined on input line 101.




LaTeX Warning: Citation `ccl-cprig-13' on page 2 undefined on input line 109.

./max_density.tex:110: Undefined control sequence.

<recently read> \xspace                         l.110 ... solution by Clark \textit{et~al.}\xspace                                                  


LaTeX Warning: Citation `ccj-udg-90' on page 2 undefined on input line 111.

[2]./max_density.tex:115: Undefined control sequence.l.115     \includegraphics                          {figs/gig}


Overfull \hbox (12.54655pt too wide) in paragraph at lines 122--127
 \OT1/cmr/bx/n/12 Mo-ti-va-tion.[] \OT1/cmr/m/n/12 Dens-est sub-graph com-pu-ta-tion on ge-o-met-ric in-ter-sec-tion graphs


LaTeX Warning: Citation `ac-ohrrt-09' on page 3 undefined on input line 138.

./max_density.tex:139: Undefined control sequence.

<recently read> \xspace                         l.139 ...he work by Afshani \textit{et~al.}\xspace                                                  


LaTeX Warning: Citation `ahz-gacor-10' on page 3 undefined on input line 140.

./max_density.tex:141: Undefined control sequence.l.141 useful for other problems.  See \hyperref                                               [sec:app-sampling]{Section~\r...

./max_density.tex:142: Undefined control sequence.l.142 \hyperref               [theo:gen-red-I]{Theorem~\ref*{theo:gen-red-I}} for details../max_density.tex:152: Undefined control sequence.l.152 approximation algorithms.  See \hyperref                                              [fig:gig]{Figure~\ref*{fig:gig}}.

[3]./max_density.tex:169: Undefined control sequence.l.169 \hyperref               [sec:expensive]{Section~\ref*{sec:expensive}} for details.  T...

./max_density.tex:172: Undefined control sequence.l.172 \hyperref               [fig:results]{Figure~\ref*{fig:results}}../max_density.tex:188: Undefined control sequence.l.188             (  \tfrac                           {1}{\varepsilon^2} + \log n)%./max_density.tex:192: Undefined control sequence.l.192         \hyperref                       [theo:first]{Theorem~\ref*{theo:first}}./max_density.tex:199: Undefined control sequence.l.199 ...  \frac{n\log^2n}{\varepsilon^2} ( \tfrac                                                  {1}{\varepsilon^2} + \log\...

./max_density.tex:203: Undefined control sequence.l.203         \hyperref                       [theo:second]{Theorem~\ref*{theo:second}}./max_density.tex:221: Undefined control sequence.l.221 statement holds \emphi                            {with high probability}, if it holds with

./max_density.tex:225: LaTeX Error: Environment observation undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.225 \begin{observation}                         

./max_density.tex:228: LaTeX Error: Environment compactenumI undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.228     \begin{compactenumI}                              

./max_density.tex:230: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.230         \item F                     or any $\varepsilon$, we have $\frac{1}{1+\varepsilon}\...



./max_density.tex:232: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.232         \item F                     or $\varepsilon \in (0,1/2)$, we have

./max_density.tex:245: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.245         \item F                     or $\varepsilon \in (0,1/3)$, we have

./max_density.tex:248: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.248         \item F                     or $\varepsilon \in (0,1)$ and constants $c, c_1$ and $...



./max_density.tex:263: LaTeX Error: \begin{document} ended by \end{compactenumI}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.263     \end{compactenumI}                            

./max_density.tex:264: LaTeX Error: \begin{document} ended by \end{observation}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.264 \end{observation}                       

./max_density.tex:266: LaTeX Error: Environment defn undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.266 \begin{defn}                  [4]./max_density.tex:267: Undefined control sequence.

<recently read> \mathbb                         l.267 ...of objects $\mathcal{D}$ (say in $\mathbb                                                  {R}^d$), their./max_density.tex:268: Undefined control sequence.l.268     \emphi                {intersection graph} has an edge between two objects if and

./max_density.tex:270: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.270     \begin{equation*}                           

./max_density.tex:271: LaTeX Error: \mathsf allowed only in math mode.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.271         \mathsf                     {G}_{\cap \mathcal{D}}./max_density.tex:271: Missing $ inserted.

<inserted text>                 $l.271         \mathsf{G}_                         {\cap \mathcal{D}}./max_density.tex:273: Undefined control sequence.l.273         \mleft                    ({\mathcal{D},./max_density.tex:274: Undefined control sequence.l.274 ...\middle\vert\; u,v \in \mathcal{D}, \text                                                  { and } u \cap v./max_density.tex:275: Undefined control sequence.l.275 ...        \neq \emptyset  \right\} }\mright                                                  ).

./max_density.tex:276: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.276     \end{equation*}                         ./max_density.tex:276: Missing $ inserted.

<inserted text>                 $l.276     \end{equation*}                         

./max_density.tex:277: LaTeX Error: \begin{document} ended by \end{defn}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.277 \end{defn}                

./max_density.tex:279: LaTeX Error: Environment defn undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.279 \begin{defn}                  ./max_density.tex:280: Undefined control sequence.l.280 ...nd a subset $S \subseteq \mathsf{V}\mleft                                                  ({\mathsf{G}}\mright)$, let./max_density.tex:280: Undefined control sequence.l.280 ...eteq \mathsf{V}\mleft({\mathsf{G}}\mright                                                  )$, let

./max_density.tex:281: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.281     \begin{equation*}                           

./max_density.tex:282: LaTeX Error: \mathsf allowed only in math mode.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.282         \mathsf                     {E}_{S}./max_density.tex:282: Missing $ inserted.

<inserted text>                 $l.282         \mathsf{E}_                         {S}./max_density.tex:284: Undefined control sequence.l.284         \mathsf{E}_{S}\mleft                                  ({\mathsf{G}}\mright)./max_density.tex:284: Undefined control sequence.l.284 ... \mathsf{E}_{S}\mleft({\mathsf{G}}\mright                                                  )./max_density.tex:286: Undefined control sequence.l.286         \left\{  uv \in \mathsf{E}\mleft                                              ({\mathsf{G}}\mright) \;\middl...

./max_density.tex:286: Undefined control sequence.l.286 ... \in \mathsf{E}\mleft({\mathsf{G}}\mright                                                  ) \;\middle\vert\; u,v \in...



./max_density.tex:287: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.287     \end{equation*}                         ./max_density.tex:287: Missing $ inserted.

<inserted text>                 $l.287     \end{equation*}                         ./max_density.tex:288: Undefined control sequence.l.288     The \emphi                    {induced subgraph} of $\mathsf{G}$ over $S$ is./max_density.tex:289: Undefined control sequence.l.289 ...athsf{E}_{S})$, and let $\mathsf{m}\mleft                                                  ({S}\mright) = \left| {\ma...

./max_density.tex:289: Undefined control sequence.l.289 ...})$, and let $\mathsf{m}\mleft({S}\mright                                                  ) = \left| {\mathsf{E}_{S}...




Overfull \hbox (34.96759pt too wide) in paragraph at lines 280--291
[]\OT1/cmr/m/n/12 For a graph $\OT1/cmss/m/n/12 G$\OT1/cmr/m/n/12 , and a sub-set $\OML/cmm/m/it/12 S \OMS/cmsy/m/n/12 ^^R \OT1/cmss/m/n/12 V\OT1/cmr/m/n/12 (\OT1/cmss/m/n/12 G\OT1/cmr/m/n/12 )$, let  E$[] = \OT1/cmss/m/n/12 E[]\OT1/cmr/m/n/12 (\OT1/cmss/m/n/12 G\OT1/cmr/m/n/12 ) = [] \OML/cmm/m/it/12 :$

./max_density.tex:292: LaTeX Error: \begin{document} ended by \end{defn}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.292 \end{defn}                

./max_density.tex:294: LaTeX Error: Environment defn undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.294 \begin{defn}                  ./max_density.tex:295: Undefined control sequence.l.295     For a set $S \subseteq \mathsf{V}\mleft                                                 ({\mathsf{G}}\mright)$, its...

./max_density.tex:295: Undefined control sequence.l.295 ...eteq \mathsf{V}\mleft({\mathsf{G}}\mright                                                  )$, its \emphi{density} in...

./max_density.tex:295: Undefined control sequence.l.295 ...}\mleft({\mathsf{G}}\mright)$, its \emphi                                                  {density} in $\mathsf{G}$ is./max_density.tex:297: Undefined control sequence.l.297         {\nabla}\mleft                            ({S}\mright) =%./max_density.tex:297: Undefined control sequence.l.297         {\nabla}\mleft({S}\mright                                       ) =%./max_density.tex:298: Undefined control sequence.l.298         \nabla_{\!\!\mathsf{G}}\mleft                                           ({S}\mright) =%./max_density.tex:298: Undefined control sequence.l.298 ... \nabla_{\!\!\mathsf{G}}\mleft({S}\mright                                                  ) =%./max_density.tex:299: Undefined control sequence.l.299         \mathsf{m}\mleft                              ({\mathsf{G}_{S}}\mright) / \left| { S} \right|,./max_density.tex:299: Undefined control sequence.l.299 ... \mathsf{m}\mleft({\mathsf{G}_{S}}\mright                                                  ) / \left| { S} \right|,./max_density.tex:301: Undefined control sequence.l.301     where $\mathsf{m}\mleft                                 ({\mathsf{G}_{S}}\mright)$ is the number of...

./max_density.tex:301: Undefined control sequence.l.301 ...$\mathsf{m}\mleft({\mathsf{G}_{S}}\mright                                                  )$ is the number of edges ...

./max_density.tex:303: Undefined control sequence.l.303     $S \subseteq \mathcal{D}$, the \emphi                                               {density} of $S$ is./max_density.tex:304: Undefined control sequence.l.304     ${\nabla}\mleft                         ({S}\mright) = \mathsf{m}\mleft({\mathsf{G}_{\cap S...

./max_density.tex:304: Undefined control sequence.l.304     ${\nabla}\mleft({S}\mright                                    ) = \mathsf{m}\mleft({\mathsf{G}_{\cap S...

./max_density.tex:304: Undefined control sequence.l.304 ...bla}\mleft({S}\mright) = \mathsf{m}\mleft                                                  ({\mathsf{G}_{\cap S}}\mri...

./max_density.tex:304: Undefined control sequence.l.304 ...hsf{m}\mleft({\mathsf{G}_{\cap S}}\mright                                                  ) / \left| { S} \right|$.

./max_density.tex:305: LaTeX Error: \begin{document} ended by \end{defn}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.305 \end{defn}                

./max_density.tex:307: LaTeX Error: Environment defn undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.307 \begin{defn}                  ./max_density.tex:308: Undefined control sequence.l.308     For a graph $\mathsf{G}$, its \emphi                                              {max density} is the quantity./max_density.tex:310: Undefined control sequence.l.310         \mathcalb                       {d}\mleft({\mathsf{G}}\mright)./max_density.tex:310: Undefined control sequence.l.310         \mathcalb{d}\mleft                                ({\mathsf{G}}\mright)./max_density.tex:310: Undefined control sequence.l.310 ...   \mathcalb{d}\mleft({\mathsf{G}}\mright                                                  )./max_density.tex:312: Undefined control sequence.l.312         = \max_{S \subseteq\mathsf{V}\mleft                                                 ({\mathsf{G}}\mright)} {\na...

./max_density.tex:312: Undefined control sequence.l.312 ...seteq\mathsf{V}\mleft({\mathsf{G}}\mright                                                  )} {\nabla}\mleft({S}\mrig...

./max_density.tex:312: Undefined control sequence.l.312 ...left({\mathsf{G}}\mright)} {\nabla}\mleft                                                  ({S}\mright),./max_density.tex:312: Undefined control sequence.l.312 ...sf{G}}\mright)} {\nabla}\mleft({S}\mright                                                  ),./max_density.tex:314: Undefined control sequence.l.314 ... set of objects $\mathcal{D}$, its \emphi                                                  {max./max_density.tex:317: Undefined control sequence.l.317         \mathcalb                       {d}\mleft({\mathcal{D}}\mright)./max_density.tex:317: Undefined control sequence.l.317         \mathcalb{d}\mleft                                ({\mathcal{D}}\mright)./max_density.tex:317: Undefined control sequence.l.317 ...  \mathcalb{d}\mleft({\mathcal{D}}\mright                                                  )./max_density.tex:319: Undefined control sequence.l.319 ...x_{S \subseteq\mathcal{D}} {\nabla}\mleft                                                  ({S}\mright),./max_density.tex:319: Undefined control sequence.l.319 ...teq\mathcal{D}} {\nabla}\mleft({S}\mright                                                  ),

./max_density.tex:321: LaTeX Error: \begin{document} ended by \end{defn}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.321 \end{defn}                


Overfull \hbox (9.04091pt too wide) in paragraph at lines 308--322
\OT1/cmr/m/n/12 and anal-o-gously, for a set of ob-jects $\OMS/cmsy/m/n/12 D$\OT1/cmr/m/n/12 , its max den-sity is $\OML/cmm/m/it/12 d\OT1/cmr/m/n/12 (\OMS/cmsy/m/n/12 D\OT1/cmr/m/n/12 ) = [][] \OMS/cmsy/m/n/12 r\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 S\OT1/cmr/m/n/12 )\OML/cmm/m/it/12 ;$


Underfull \hbox (badness 10000) in paragraph at lines 308--322


./max_density.tex:325: Undefined control sequence.l.325 then it is the \emphi                           {densest subset} of $\mathcal{D}$ (i.e.,./max_density.tex:326: Undefined control sequence.

<recently read> \mleft                        l.326 $\mleft             ({\mathsf{G}_{\cap \mathcal{D}}}\mright)_{S}$ is the densest su...

./max_density.tex:326: Undefined control sequence.l.326 ...ft({\mathsf{G}_{\cap \mathcal{D}}}\mright                                                  )_{S}$ is the densest subg...



./max_density.tex:332: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.332 \begin{lemma}                   ./max_density.tex:336: Undefined control sequence.l.336     $\nabla = {\nabla}\mleft                                  ({\mathcal{O}}\mright)$. Then, for any obj...

./max_density.tex:336: Undefined control sequence.l.336 ...bla = {\nabla}\mleft({\mathcal{O}}\mright                                                  )$. Then, for any object $...

./max_density.tex:337: Undefined control sequence.l.337     have $d_{\mathcal{O}}\mleft                                     ({u}\mright) = \left| { u \sqcap (\math...

./max_density.tex:337: Undefined control sequence.l.337     have $d_{\mathcal{O}}\mleft({u}\mright                                                ) = \left| { u \sqcap (\math...



./max_density.tex:341: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.341 \end{lemma}                 

./max_density.tex:342: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.342 \begin{proof}                   

./max_density.tex:344: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.344     \begin{equation*}                           ./max_density.tex:345: Missing $ inserted.

<inserted text>                 $l.345         \nabla                    ./max_density.tex:349: Undefined control sequence.

<argument> ...} \right | + d_{\mathcal {O}}\mleft                                                   ({u}\mright )l.349 ...ht)}{\left| {\mathcal{O}} \right| -1 + 1}                                                  ../max_density.tex:349: Undefined control sequence.

<argument> ... d_{\mathcal {O}}\mleft ({u}\mright                                                   )l.349 ...ht)}{\left| {\mathcal{O}} \right| -1 + 1}                                                  .

./max_density.tex:350: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.350     \end{equation*}                         ./max_density.tex:350: Missing $ inserted.

<inserted text>                 $l.350     \end{equation*}                         ./max_density.tex:351: Undefined control sequence.l.351     As such, if $d_{\mathcal{O}}\mleft                                            ({u}\mright) < \nabla$, then./max_density.tex:351: Undefined control sequence.l.351 ...uch, if $d_{\mathcal{O}}\mleft({u}\mright                                                  ) < \nabla$, then

./max_density.tex:352: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.352     \begin{equation*}                           ./max_density.tex:353: Missing $ inserted.

<inserted text>                 $l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:353: Undefined control sequence.

<argument> d_{\mathcal {O}}\mleft                                   ({u}\mright )l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:353: Undefined control sequence.

<argument> d_{\mathcal {O}}\mleft ({u}\mright                                               )l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:353: Missing $ inserted.

<inserted text>                 $l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:353: Missing $ inserted.

<inserted text>                 $l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:353: Extra }, or forgotten $.\frac  #1#2->{\begingroup #1\endgroup \over #2}                                               l.353 ...rac{d_{\mathcal{O}}\mleft({u}\mright)}{1}                                                  ./max_density.tex:357: Undefined control sequence.

<argument> d_{\mathcal {O}}\mleft                                   ({u}\mright ) + \left | {\mathsf {E}_{\mat...l.357 ...t|}{1 + \left| {\mathcal{O}} \right| -1 }                                                  ./max_density.tex:357: Undefined control sequence.

<argument> d_{\mathcal {O}}\mleft ({u}\mright                                               ) + \left | {\mathsf {E}_{\mat...l.357 ...t|}{1 + \left| {\mathcal{O}} \right| -1 }                                                  

./max_density.tex:360: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.360     \end{equation*}                         ./max_density.tex:360: Missing $ inserted.

<inserted text>                 $l.360     \end{equation*}                         ./max_density.tex:360: Missing } inserted.

<inserted text>                 }l.360     \end{equation*}                         

./max_density.tex:363: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.363 \end{proof}                 ./max_density.tex:367: Undefined control sequence.l.367 The algorithm of \hyperref                                [sec:expensive]{Section~\ref*{sec:expensive}...



./max_density.tex:369: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.369 \begin{lemma}                   

./max_density.tex:375: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.375 \end{lemma}                 

./max_density.tex:376: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.376 \begin{proof}                   ./max_density.tex:383: Undefined control sequence.l.383     $\mathcal{A}\mleft                            ({\mathcal{D}}\mright)$ can be done in./max_density.tex:383: Undefined control sequence.l.383     $\mathcal{A}\mleft({\mathcal{D}}\mright                                                 )$ can be done in


LaTeX Warning: Citation `h-gaa-11' on page 5 undefined on input line 384.

./max_density.tex:385: Undefined control sequence.l.385     \hyperref                   [fig:vert-dec]{Figure~\ref*{fig:vert-dec}} for an[5]

./max_density.tex:414: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.414 \end{proof}                 ./max_density.tex:418: Undefined control sequence.l.418     \includegraphics                          {figs/vert_dec}./max_density.tex:418: Missing $ inserted.

<inserted text>                 $l.418     \includegraphics{figs/vert_                                     dec}./max_density.tex:418: Extra }, or forgotten $.l.418     \includegraphics{figs/vert_dec}                                         ./max_density.tex:419: Missing $ inserted.

<inserted text>                 $l.419 ...on{Vertical decomposition of four disks.}                                                  ./max_density.tex:421: Missing } inserted.

<inserted text>                 }l.421 \end{figure}                  


Overfull \hbox (61.43768pt too wide) in paragraph at lines 423--423
[]\OT1/cmr/bx/n/17.28 From re-port-ing to ap-prox-i-mate sam-pling/counting [6]

./max_density.tex:451: LaTeX Error: Environment example undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.451 \begin{example}                     


LaTeX Warning: Citation `l-nopkn-22' on page 7 undefined on input line 454.



./max_density.tex:458: LaTeX Error: \begin{document} ended by \end{example}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.458 \end{example}                   


Overfull \hbox (22.52176pt too wide) in paragraph at lines 480--507
\OT1/cmr/m/n/12 structure as-so-ci-ated with each node, to find the max-i-mal $\OML/cmm/m/it/12 i$\OT1/cmr/m/n/12 , such that $[] \OML/cmm/m/it/12 >[7]

./max_density.tex:511: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.511 \begin{lemma}                   ./max_density.tex:524: Undefined control sequence.l.524         {\mathbb                      {P}}\mleft[ \Bigl.\smash{\left| {\mathcal{D}(v) \sqcap...

./max_density.tex:524: Undefined control sequence.l.524         {\mathbb{P}}\mleft                                [ \Bigl.\smash{\left| {\mathcal{D}(v) \sqcap...

./max_density.tex:525: Undefined control sequence.l.525 ...\sqcap \mathsf{q}} \right|}{2^i}} \mright                                                  ]

./max_density.tex:529: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.529 \end{lemma}                 

./max_density.tex:530: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.530 \begin{proof}                   Consider a node $v$ at a distance $i$ from the root, and./max_density.tex:532: Undefined control sequence.l.532     $\mu_v = {\mathbb                           {E}}\mleft[ Y_v \mright] = \left| { \mathcal{D} \...

./max_density.tex:532: Undefined control sequence.l.532     $\mu_v = {\mathbb{E}}\mleft                                     [ Y_v \mright] = \left| { \mathcal{D} \...

./max_density.tex:532: Undefined control sequence.l.532     $\mu_v = {\mathbb{E}}\mleft[ Y_v \mright                                                  ] = \left| { \mathcal{D} \...

./max_density.tex:534: Undefined control sequence.l.534     \hyperref                   [theo:special:h:i:e]{Chernoff's inequality}, we have

./max_density.tex:535: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.535     \begin{equation*}                           ./max_density.tex:536: Undefined control sequence.l.536         {\mathbb                      {P}}\mleft[ \bigl. Y_v \notin (1\pm \varepsilon/2)\mu_...

./max_density.tex:536: Undefined control sequence.l.536         {\mathbb{P}}\mleft                                [ \bigl. Y_v \notin (1\pm \varepsilon/2)\mu_...

./max_density.tex:536: Missing $ inserted.

<inserted text>                 $l.536         {\mathbb{P}}\mleft[ \bigl                                       . Y_v \notin (1\pm \varepsilon/2)\mu_...

./max_density.tex:536: Undefined control sequence.l.536 ... \notin (1\pm \varepsilon/2)\mu_v \mright                                                  ]./max_density.tex:538: Undefined control sequence.l.538         2\exp\mleft                         ({ - \varepsilon^2 \mu_v /3 }\mright)./max_density.tex:538: Undefined control sequence.l.538 ...mleft({ - \varepsilon^2 \mu_v /3 }\mright                                                  )./max_density.tex:540: Undefined control sequence.l.540         2\exp\mleft                         ({ - \varepsilon^2 \psi_\varepsilon /48 }\mright)./max_density.tex:540: Undefined control sequence.l.540 ...arepsilon^2 \psi_\varepsilon /48 }\mright                                                  )./max_density.tex:542: Undefined control sequence.l.542         2\exp\mleft                         ({ - (c/48)\log n }\mright)./max_density.tex:542: Undefined control sequence.l.542 ...    2\exp\mleft({ - (c/48)\log n }\mright                                                  )

./max_density.tex:545: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.545     \end{equation*}                         ./max_density.tex:545: Missing $ inserted.

<inserted text>                 $l.545     \end{equation*}                         ./max_density.tex:549: Undefined control sequence.l.549     ${\mathbb                   {P}}\mleft[ Y_v \notin (1\pm \varepsilon/2)\mu_v \mright]...

./max_density.tex:549: Undefined control sequence.l.549     ${\mathbb{P}}\mleft                             [ Y_v \notin (1\pm \varepsilon/2)\mu_v \mright]...

./max_density.tex:549: Undefined control sequence.l.549 ... \notin (1\pm \varepsilon/2)\mu_v \mright                                                  ] \leq {1}/{n^{\Omega(c)}}$.

./max_density.tex:550: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.550 \end{proof}                 

./max_density.tex:552: LaTeX Error: Environment observation undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.552 \begin{observation}                         ./max_density.tex:555: Undefined control sequence.l.555     \hyperref                   [lemma:a:high:is:good]{Lemma~\ref*{lemma:a:high:is:good}}./max_density.tex:559: Undefined control sequence.l.559         {\mathbb                      {P}}\mleft[ \bigl.\left| {\mathcal{D}(v) \sqcap \maths...

./max_density.tex:559: Undefined control sequence.l.559         {\mathbb{P}}\mleft                                [ \bigl.\left| {\mathcal{D}(v) \sqcap \maths...

./max_density.tex:559: Undefined control sequence.l.559 ...{q}} \right| > \psi_{\varepsilon} \mright                                                  ]./max_density.tex:562: Undefined control sequence.l.562     Indeed, \hyperref                           [lemma:a:high:is:good]{Lemma~\ref*{lemma:a:high:i...



./max_density.tex:565: LaTeX Error: \begin{document} ended by \end{observation}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.565 \end{observation}                       

./max_density.tex:567: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.567 \begin{lemma}                   

./max_density.tex:578: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.578 \end{lemma}                 

./max_density.tex:579: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.579 \begin{proof}                   ./max_density.tex:584: Undefined control sequence.l.584     n$. By \hyperref                          [observation:low:is:small]{Observation~\ref*{obser...

./max_density.tex:585: Undefined control sequence.l.585     $j\leq M$. By \hyperref                                 [lemma:a:high:is:good]{Lemma~\ref*{lemma:a:...



./max_density.tex:593: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.593     \begin{equation*}                           ./max_density.tex:594: Missing $ inserted.

<inserted text>                 $l.594         \frac{1-\varepsilon}{\beta}                                         ./max_density.tex:594: Missing $ inserted.

<inserted text>                 $l.594         \frac{1-\varepsilon}{\beta}                                         ./max_density.tex:594: Missing $ inserted.

<inserted text>                 $l.594         \frac{1-\varepsilon}{\beta}                                         ./max_density.tex:594: Extra }, or forgotten $.\frac  #1#2->{\begingroup #1\endgroup \over #2}                                               l.594         \frac{1-\varepsilon}{\beta}                                         

./max_density.tex:606: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.606     \end{equation*}                         ./max_density.tex:606: Missing $ inserted.

<inserted text>                 $l.606     \end{equation*}                         ./max_density.tex:606: Missing } inserted.

<inserted text>                 }l.606     \end{equation*}                         ./max_density.tex:611: Undefined control sequence.l.611     \hyperref                   [lemma:a:high:is:good]{Lemma~\ref*{lemma:a:high:is:good}}.

./max_density.tex:612: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.612 \end{proof}                 [8]

./max_density.tex:623: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.623 \begin{equation*}                       ./max_density.tex:624: Missing $ inserted.

<inserted text>                 $l.624     \tau              ./max_density.tex:626: Undefined control sequence.l.626     {\mathbb                  {E}}\mleft[ \Bigl.\smash{\sum\nolimits_{t=j}^i} O( Q(n) + ...

./max_density.tex:626: Undefined control sequence.l.626     {\mathbb{E}}\mleft                            [ \Bigl.\smash{\sum\nolimits_{t=j}^i} O( Q(n) + ...

./max_density.tex:627: Undefined control sequence.l.627 ...      \sqcap \mathsf{q}} \right|) \mright                                                  ].

./max_density.tex:628: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.628 \end{equation*}                     ./max_density.tex:628: Missing $ inserted.

<inserted text>                 $l.628 \end{equation*}                     

./max_density.tex:630: LaTeX Error: Environment compactenumA undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.630 \begin{compactenumA}                          

./max_density.tex:632: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.632     \item I                 f $Q(n) = O(\log n)$, then $\tau = O( \psi_\varepsilon)$, a...



./max_density.tex:639: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.639     \item I                 f $Q(n)=\Omega(\log n)$, we have (in expectation) that

./max_density.tex:644: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.644     \item I                 f $Q(n)=O(n^{\lambda})$, for $0< \lambda \leq 1$, then the

./max_density.tex:648: LaTeX Error: \begin{document} ended by \end{compactenumA}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.648 \end{compactenumA}                        ./max_density.tex:652: Undefined control sequence.l.652 \emphw            {well-behaved}, if for any non-negative integers

./max_density.tex:660: LaTeX Error: Environment theorem undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.660 \begin{theorem}                     %

./max_density.tex:675: LaTeX Error: Environment compactenumi undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.675     \begin{compactenumi}                              

./max_density.tex:677: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.677         \item $                     O( (\varepsilon^{-2} + \log \log n) \log n)$ if[9]

./max_density.tex:681: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.681         \item $                     O( Q(n))$ if $Q(m) =O(m^{\lambda})$, for some constant

./max_density.tex:686: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.686         $               O\bigl( \varepsilon^{-2} \log n + Q(n) \log \tfrac{\log n}{\v...

./max_density.tex:686: Undefined control sequence.l.686 ...varepsilon^{-2} \log n + Q(n) \log \tfrac                                                  {\log n}{\varepsilon} )$

./max_density.tex:688: LaTeX Error: \begin{document} ended by \end{compactenumi}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.688     \end{compactenumi}                            

./max_density.tex:689: LaTeX Error: \begin{document} ended by \end{theorem}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.689 \end{theorem}                   


LaTeX Warning: Citation `l-nopkn-22' on page 10 undefined on input line 691.




Overfull \hbox (9.32516pt too wide) in paragraph at lines 691--694
[]\OT1/cmr/m/n/12 Plugging in the data-structure of Liu [[]] for disks, with $\OML/cmm/m/it/12 C\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 m\OT1/cmr/m/n/12 ) = \OML/cmm/m/it/12 O\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 m [] m\OT1/cmr/m/n/12 )$,

./max_density.tex:695: LaTeX Error: Environment corollary undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.695 \begin{corollary}                       \label{cor:disks-estimate}

./max_density.tex:705: LaTeX Error: \begin{document} ended by \end{corollary}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.705 \end{corollary}                     ./max_density.tex:717: Undefined control sequence.

<recently read> \mathcalb                           l.717 ... values to the optimal density $\mathcalb                                                  {d}$. To this./max_density.tex:718: Undefined control sequence.l.718 end, in the $i$th\xspace                               round, the algorithm would try the degree thr...



./max_density.tex:724: LaTeX Error: Environment compactenumI undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.724 \begin{compactenumI}                          [itemsep=-0.5ex]

./max_density.tex:726: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.726     \item T                 he algorithm constructs the data-structure of./max_density.tex:727: Undefined control sequence.l.727     \hyperref                   [cor:disks-estimate]{Corollary~\ref*{cor:disks-estimate}}...




Overfull \hbox (19.35269pt too wide) in paragraph at lines 726--728
[]\OT1/cmr/m/n/12 The al-go-rithm con-structs the data-structure of [cor:disks-estimate]Corollary 3.2.3[]

./max_density.tex:729: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.729     \item L                 et $\mathcal{L}_< \subseteq \mathcal{L}$ be the objects who...



./max_density.tex:733: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.733     \item I                 f $\mathcal{L}_\geq$ is empty, then this round failed, and the



./max_density.tex:736: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.736     \item I                 f $\left| {L_{<}} \right| < \vartheta \left| {\mathcal{L}} ...



./max_density.tex:739: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.739     \item O                 therwise, let $\mathcal{L} \leftarrow \mathcal{L} \setminus...



./max_density.tex:742: LaTeX Error: \begin{document} ended by \end{compactenumI}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.742 \end{compactenumI}                        [10]

./max_density.tex:746: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.746 \begin{lemma}                   ./max_density.tex:750: Undefined control sequence.l.750     $\beta \geq (1-\vartheta)^3\mathcalb                                              {d}$, with high probability, w...

./max_density.tex:751: Undefined control sequence.

<recently read> \mathcalb                           l.751     $\mathcalb                    {d}$ is the optimal density.

./max_density.tex:752: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.752 \end{lemma}                 

./max_density.tex:753: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.753 \begin{proof}                   ./max_density.tex:755: Undefined control sequence.l.755     $\beta \in [(1-\vartheta)^3\mathcalb                                              {d}, (1-\vartheta)^2\mathcalb{...

./max_density.tex:755: Undefined control sequence.l.755 ...)^3\mathcalb{d}, (1-\vartheta)^2\mathcalb                                                  {d}]$. By definition of./max_density.tex:757: Undefined control sequence.l.757 ...leq (1+\vartheta)(1-\vartheta)^2\mathcalb                                                  {d}\leq./max_density.tex:758: Undefined control sequence.l.758     (1-\vartheta)\mathcalb                                {d}$.  By \hyperref[lemma:density:l:b]{Lemma...

./max_density.tex:758: Undefined control sequence.l.758 ...(1-\vartheta)\mathcalb{d}$.  By \hyperref                                                  [lemma:density:l:b]{Lemma~...

./max_density.tex:759: Undefined control sequence.l.759 ...imal solution have degree $\geq \mathcalb                                                  {d}$ (when restricted to the

./max_density.tex:766: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.766 \end{proof}                 

./max_density.tex:767: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.767 \begin{lemma}                   

./max_density.tex:772: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.772 \end{lemma}                 

./max_density.tex:773: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.773 \begin{proof}                   ./max_density.tex:776: Undefined control sequence.l.776     \hyperref                   [lemma:beta-at-least]{Lemma~\ref*{lemma:beta-at-least}}, ...

./max_density.tex:776: Undefined control sequence.l.776 ...t}}, $\beta \geq (1-\vartheta)^3\mathcalb                                                  {d}$, and by the

./max_density.tex:783: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.783     \begin{equation*}                           

./max_density.tex:784: LaTeX Error: \mathsf allowed only in math mode.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.784         \mathsf                     {m}\mleft({\mathcal{L}}\mright)./max_density.tex:784: Undefined control sequence.l.784         \mathsf{m}\mleft                              ({\mathcal{L}}\mright)

./max_density.tex:784: LaTeX Error: \mathcal allowed only in math mode.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.784         \mathsf{m}\mleft({\mathcal                                        {L}}\mright)./max_density.tex:784: Undefined control sequence.l.784 ...    \mathsf{m}\mleft({\mathcal{L}}\mright                                                  )./max_density.tex:785: Missing $ inserted.

<inserted text>                 $l.785         \geq                  ./max_density.tex:790: Undefined control sequence.

<argument> \mathcalb                      {d}l.790 ...    (1-\vartheta)^5\frac{\mathcalb{d}}{2}                                                   \left| {\mathcal{L}} \right|

./max_density.tex:792: Undefined control sequence.

<argument> \mathcalb                      {d}l.792 ...    (1-5\vartheta) \frac{\mathcalb{d}}{2}                                                   \left| {\mathcal{L}} \rig...



./max_density.tex:793: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.793     \end{equation*}                         ./max_density.tex:793: Missing $ inserted.

<inserted text>                 $l.793     \end{equation*}                         ./max_density.tex:795: Undefined control sequence.l.795     ${\nabla}\mleft                         ({\mathcal{L}}\mright) = \frac{\mathsf{m}\mleft({\m...

./max_density.tex:795: Undefined control sequence.l.795     ${\nabla}\mleft({\mathcal{L}}\mright                                              ) = \frac{\mathsf{m}\mleft({\m...

./max_density.tex:795: Undefined control sequence.

<argument> \mathsf {m}\mleft                              ({\mathcal {L}}\mright )l.795 ...}}\mright)}{\left| {\mathcal{L}} \right|}                                                   \geq (1-5 \vartheta)./max_density.tex:795: Undefined control sequence.

<argument> ...sf {m}\mleft ({\mathcal {L}}\mright                                                   )l.795 ...}}\mright)}{\left| {\mathcal{L}} \right|}                                                   \geq (1-5 \vartheta)./max_density.tex:796: Undefined control sequence.l.796     \mathcalb                   {d}/2 = (1-\varepsilon/3)\mathcalb{d}/2$, as $\vartheta= ...

./max_density.tex:796: Undefined control sequence.l.796 ...athcalb{d}/2 = (1-\varepsilon/3)\mathcalb                                                  {d}/2$, as $\vartheta= \va...



./max_density.tex:798: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.798 \end{proof}                 

./max_density.tex:800: LaTeX Error: Environment theorem undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.800 \begin{theorem}                     

./max_density.tex:809: LaTeX Error: \begin{document} ended by \end{theorem}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.809 \end{theorem}                   

./max_density.tex:810: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.810 \begin{proof}                   

./max_density.tex:829: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.829 \end{proof}                 [11]./max_density.tex:843: Undefined control sequence.

<recently read> \mathcalb                           l.843 maximum subgraph density $\mathcalb                                         {d}$. Let $\vartheta \in (0,1/6)$ be a



./max_density.tex:846: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.846 \begin{equation*}                       ./max_density.tex:847: Undefined control sequence.l.847     \mathcalb                   {d}./max_density.tex:849: Undefined control sequence.l.849     \mathcalb                   {d}\mleft({\mathsf{G}}\mright)./max_density.tex:849: Undefined control sequence.l.849     \mathcalb{d}\mleft                            ({\mathsf{G}}\mright)

./max_density.tex:849: LaTeX Error: \mathsf allowed only in math mode.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.849     \mathcalb{d}\mleft({\mathsf                                     {G}}\mright)./max_density.tex:849: Undefined control sequence.l.849     \mathcalb{d}\mleft({\mathsf{G}}\mright                                                )./max_density.tex:850: Missing $ inserted.

<inserted text>                 $l.850     \geq              

./max_density.tex:854: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.854 \end{equation*}                     ./max_density.tex:854: Missing $ inserted.

<inserted text>                 $l.854 \end{equation*}                     

./max_density.tex:857: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.857 \begin{equation*}                       ./max_density.tex:858: Missing $ inserted.

<inserted text>                 $l.858     \psi              

./max_density.tex:867: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.867 \end{equation*}                     ./max_density.tex:867: Missing $ inserted.

<inserted text>                 $l.867 \end{equation*}                     ./max_density.tex:870: Undefined control sequence.l.870 $i$th\xspace                   iteration, an edge $e_i$ is picked from the graph, where the




LaTeX Warning: Citation `mtvv-dsdgs-15' on page 12 undefined on input line 876.



./max_density.tex:881: Undefined control sequence.l.881 summarized in \hyperref                             [lemma:sampling]{Lemma~\ref*{lemma:sampling}}, ...



./max_density.tex:886: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.886 \begin{lemma}                   ./max_density.tex:889: Undefined control sequence.

<recently read> \mathcalb                           l.889     Let $\mathcalb                        {d} = \mathcalb{d}\mleft({\mathsf{G}}\mright)$, and ...

./max_density.tex:889: Undefined control sequence.l.889     Let $\mathcalb{d} = \mathcalb                                       {d}\mleft({\mathsf{G}}\mright)$, and ...

./max_density.tex:889: Undefined control sequence.l.889     Let $\mathcalb{d} = \mathcalb{d}\mleft                                                ({\mathsf{G}}\mright)$, and ...

./max_density.tex:889: Undefined control sequence.l.889 ... = \mathcalb{d}\mleft({\mathsf{G}}\mright                                                  )$, and let $U \subseteq V...

./max_density.tex:890: Undefined control sequence.l.890 ...tices.  If $\nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright) \leq \mathcal...

./max_density.tex:890: Undefined control sequence.l.890 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \leq \mathcalb{d}/60$, then

./max_density.tex:890: Undefined control sequence.l.890 ...thsf{G}}\mleft({U}\mright) \leq \mathcalb                                                  {d}/60$, then./max_density.tex:891: Undefined control sequence.l.891     ${\mathbb                   {P}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright) \geq \psi \m...

./max_density.tex:891: Undefined control sequence.l.891     ${\mathbb{P}}\mleft                             [ \nabla_{\!\!H}\mleft({U}\mright) \geq \psi \m...

./max_density.tex:891: Undefined control sequence.l.891 ...${\mathbb{P}}\mleft[ \nabla_{\!\!H}\mleft                                                  ({U}\mright) \geq \psi \ma...

./max_density.tex:891: Undefined control sequence.l.891 ...}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright                                                  ) \geq \psi \mathcalb{d} /...

./max_density.tex:891: Undefined control sequence.l.891 ...!H}\mleft({U}\mright) \geq \psi \mathcalb                                                  {d} /5  \mright] \leq n^{-...

./max_density.tex:891: Undefined control sequence.l.891 ...right) \geq \psi \mathcalb{d} /5  \mright                                                  ] \leq n^{-100k}$.

./max_density.tex:892: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.892 \end{lemma}                 

./max_density.tex:893: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.893 \begin{proof}                   ./max_density.tex:894: Undefined control sequence.

<recently read> \mathcalb                           l.894     We have $\mathcalb                            {d} \geq m/ n$, where $n = \left| {\mathsf{V}\ml...

./max_density.tex:894: Undefined control sequence.l.894 .../ n$, where $n = \left| {\mathsf{V}\mleft                                                  ({\mathsf{G}}\mright)} \ri...

./max_density.tex:894: Undefined control sequence.l.894 ...ft| {\mathsf{V}\mleft({\mathsf{G}}\mright                                                  )} \right|$ and./max_density.tex:895: Undefined control sequence.l.895     $m = \left| {\mathsf{E}\mleft                                       ({ \mathsf{G}}\mright)} \right|$, and...

./max_density.tex:895: Undefined control sequence.l.895 ...t| {\mathsf{E}\mleft({ \mathsf{G}}\mright                                                  )} \right|$, and thus

./max_density.tex:896: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.896     \begin{equation*}                           ./max_density.tex:897: Missing $ inserted.

<inserted text>                 $l.897         \psi                  ./max_density.tex:903: Undefined control sequence.

<argument> \mathcalb                      {d}l.903         \frac{1}{\mathcalb{d}}                                     \cdot  \frac{c}{(1+\vartheta) \vartheta...



./max_density.tex:904: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.904     \end{equation*}                         ./max_density.tex:904: Missing $ inserted.

<inserted text>                 $l.904     \end{equation*}                         ./max_density.tex:905: Undefined control sequence.l.905 ...$ if the edge sampled in the $i$th\xspace                                                   round belongs to

./max_density.tex:908: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.908     \begin{equation*}                           ./max_density.tex:909: Undefined control sequence.l.909         {\mathbb                      {P}}\mleft[ X_i=1 \mright]./max_density.tex:909: Undefined control sequence.l.909         {\mathbb{P}}\mleft                                [ X_i=1 \mright]./max_density.tex:909: Missing $ inserted.

<inserted text>                 $l.909         {\mathbb{P}}\mleft[ X_                                    i=1 \mright]./max_density.tex:909: Undefined control sequence.l.909         {\mathbb{P}}\mleft[ X_i=1 \mright                                               ]./max_density.tex:911: Undefined control sequence.

<argument> \left | {\mathsf {E}\mleft                                       ({\mathsf {G}_{U}}\mright )} \right |l.911 ...eft({\mathsf{G}_{U}}\mright)} \right|}{m}                                                  ./max_density.tex:911: Undefined control sequence.

<argument> ...{E}\mleft ({\mathsf {G}_{U}}\mright                                                   )} \right |l.911 ...eft({\mathsf{G}_{U}}\mright)} \right|}{m}                                                  ./max_density.tex:913: Undefined control sequence.

<argument> k \nabla _{\!\!\mathsf {G}}\mleft                                              ({U}\mright )l.913 ...la_{\!\!\mathsf{G}}\mleft({U}\mright)}{m}                                                  ../max_density.tex:913: Undefined control sequence.

<argument> ...{\!\!\mathsf {G}}\mleft ({U}\mright                                                   )l.913 ...la_{\!\!\mathsf{G}}\mleft({U}\mright)}{m}                                                  .

./max_density.tex:914: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.914     \end{equation*}                         ./max_density.tex:914: Missing $ inserted.

<inserted text>                 $l.914     \end{equation*}                         [12]./max_density.tex:918: Undefined control sequence.l.918         {\mathbb                      {E}}\mleft[ X \mright]%./max_density.tex:918: Undefined control sequence.l.918         {\mathbb{E}}\mleft                                [ X \mright]%./max_density.tex:918: Undefined control sequence.l.918         {\mathbb{E}}\mleft[ X \mright                                           ]%./max_density.tex:920: Undefined control sequence.

<argument> k \nabla _{\!\!\mathsf {G}}\mleft                                              ({U}\mright )l.920 ...la_{\!\!\mathsf{G}}\mleft({U}\mright)}{m}                                                  %./max_density.tex:920: Undefined control sequence.

<argument> ...{\!\!\mathsf {G}}\mleft ({U}\mright                                                   )l.920 ...la_{\!\!\mathsf{G}}\mleft({U}\mright)}{m}                                                  %./max_density.tex:922: Undefined control sequence.l.922 ...a)^2 \psi k \nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright)../max_density.tex:922: Undefined control sequence.l.922 ... \nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  )../max_density.tex:926: Undefined control sequence.l.926 ...assumption $\nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright) \leq \mathcal...

./max_density.tex:926: Undefined control sequence.l.926 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \leq \mathcalb{d}/60$, i...

./max_density.tex:926: Undefined control sequence.l.926 ...thsf{G}}\mleft({U}\mright) \leq \mathcalb                                                  {d}/60$, implying that./max_density.tex:927: Undefined control sequence.l.927     ${\mathbb                   {E}}\mleft[ X \mright] \leq (1+3\vartheta) \psi k \mathca...

./max_density.tex:927: Undefined control sequence.l.927     ${\mathbb{E}}\mleft                             [ X \mright] \leq (1+3\vartheta) \psi k \mathca...

./max_density.tex:927: Undefined control sequence.l.927     ${\mathbb{E}}\mleft[ X \mright                                        ] \leq (1+3\vartheta) \psi k \mathca...

./max_density.tex:927: Undefined control sequence.l.927 ...ght] \leq (1+3\vartheta) \psi k \mathcalb                                                  {d}/60 \leq \psi k \mathca...

./max_density.tex:927: Undefined control sequence.l.927 ...i k \mathcalb{d}/60 \leq \psi k \mathcalb                                                  {d}/30$, if./max_density.tex:928: Undefined control sequence.l.928     $\vartheta \in (0,1/3)$, by \hyperref                                               [observation:eps:games]{Obser...

./max_density.tex:930: Undefined control sequence.l.930         (1+ (2e-1)){\mathbb                                 {E}}\mleft[ X \mright] \leq \frac{\psi k \m...

./max_density.tex:930: Undefined control sequence.l.930         (1+ (2e-1)){\mathbb{E}}\mleft                                           [ X \mright] \leq \frac{\psi k \m...

./max_density.tex:930: Undefined control sequence.l.930 ... (1+ (2e-1)){\mathbb{E}}\mleft[ X \mright                                                  ] \leq \frac{\psi k \mathc...

./max_density.tex:930: Undefined control sequence.

<argument> \psi k \mathcalb                             {d}l.930 ...right] \leq \frac{\psi k \mathcalb{d}}{5}                                                  ../max_density.tex:932: Undefined control sequence.l.932     By Chernoff's inequality, \hyperref                                             [lemma:chernoff:delta:big]{Lemm...




Overfull \hbox (72.58008pt too wide) in paragraph at lines 925--933
\OT1/cmr/m/n/12 that $(1 + (2\OML/cmm/m/it/12 e \OMS/cmsy/m/n/12 ^^@ \OT1/cmr/m/n/12 1))\OML/cmm/m/it/12 E\OT1/cmr/m/n/12 [\OML/cmm/m/it/12 X\OT1/cmr/m/n/12 ] \OMS/cmsy/m/n/12 ^^T []\OML/cmm/m/it/12 :$ \OT1/cmr/m/n/12 By Cher-noff's in-equal-ity, [lemma:chernoff:delta:big]Lemma A[],

./max_density.tex:934: LaTeX Error: Environment align* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.934     \begin{align*}                        ./max_density.tex:935: Undefined control sequence.l.935       {\mathbb                    {P}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright) \geq \frac{...

./max_density.tex:935: Undefined control sequence.l.935       {\mathbb{P}}\mleft                              [ \nabla_{\!\!H}\mleft({U}\mright) \geq \frac{...

./max_density.tex:935: Missing $ inserted.

<inserted text>                 $l.935       {\mathbb{P}}\mleft[ \nabla                                      _{\!\!H}\mleft({U}\mright) \geq \frac{...

./max_density.tex:935: Undefined control sequence.l.935 ... {\mathbb{P}}\mleft[ \nabla_{\!\!H}\mleft                                                  ({U}\mright) \geq \frac{\p...

./max_density.tex:935: Undefined control sequence.l.935 ...}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright                                                  ) \geq \frac{\psi \mathcal...

./max_density.tex:935: Undefined control sequence.

<argument> \psi \mathcalb                           {d}l.935 ...\mright) \geq \frac{\psi \mathcalb{d}}{5}                                                   \mright]./max_density.tex:935: Undefined control sequence.l.935 ... \geq \frac{\psi \mathcalb{d}}{5} \mright                                                  ]./max_density.tex:936: Misplaced alignment tab character &.l.936       &             =./max_density.tex:937: Undefined control sequence.l.937         {\mathbb                      {P}}\mleft[ X \geq \frac{\psi k \mathcalb{d}}{ 5} \mri...

./max_density.tex:937: Undefined control sequence.l.937         {\mathbb{P}}\mleft                                [ X \geq \frac{\psi k \mathcalb{d}}{ 5} \mri...

./max_density.tex:937: Undefined control sequence.

<argument> \psi k \mathcalb                             {d}l.937 ...ft[ X \geq \frac{\psi k \mathcalb{d}}{ 5}                                                   \mright]./max_density.tex:937: Undefined control sequence.l.937 ...eq \frac{\psi k \mathcalb{d}}{ 5} \mright                                                  ]./max_density.tex:939: Undefined control sequence.l.939         2^{-\psi k \mathcalb                                  {d}/5}

./max_density.tex:942: LaTeX Error: \begin{document} ended by \end{align*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.942     \end{align*}                      ./max_density.tex:942: Missing $ inserted.

<inserted text>                 $l.942     \end{align*}                      

./max_density.tex:944: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.944 \end{proof}                 

./max_density.tex:946: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.946 \begin{lemma}                   ./max_density.tex:949: Undefined control sequence.

<recently read> \mathcalb                           l.949     Let $\mathcalb                        {d} = \mathcalb{d}\mleft({\mathsf{G}}\mright)$, and ...

./max_density.tex:949: Undefined control sequence.l.949     Let $\mathcalb{d} = \mathcalb                                       {d}\mleft({\mathsf{G}}\mright)$, and ...

./max_density.tex:949: Undefined control sequence.l.949     Let $\mathcalb{d} = \mathcalb{d}\mleft                                                ({\mathsf{G}}\mright)$, and ...

./max_density.tex:949: Undefined control sequence.l.949 ... = \mathcalb{d}\mleft({\mathsf{G}}\mright                                                  )$, and let $U \subseteq V...

./max_density.tex:950: Undefined control sequence.l.950 ...tices.  If $\nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright) \geq \mathcal...

./max_density.tex:950: Undefined control sequence.l.950 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \geq \mathcalb{d}/60$, then

./max_density.tex:950: Undefined control sequence.l.950 ...thsf{G}}\mleft({U}\mright) \geq \mathcalb                                                  {d}/60$, then./max_density.tex:951: Undefined control sequence.l.951     ${\mathbb                   {P}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright) \in (1\pm \v...

./max_density.tex:951: Undefined control sequence.l.951     ${\mathbb{P}}\mleft                             [ \nabla_{\!\!H}\mleft({U}\mright) \in (1\pm \v...

./max_density.tex:951: Undefined control sequence.l.951 ...${\mathbb{P}}\mleft[ \nabla_{\!\!H}\mleft                                                  ({U}\mright) \in (1\pm \va...

./max_density.tex:951: Undefined control sequence.l.951 ...}}\mleft[ \nabla_{\!\!H}\mleft({U}\mright                                                  ) \in (1\pm \vartheta)^3 \...

./max_density.tex:951: Undefined control sequence.l.951 ...eta)^3 \psi \nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright)  \mright]./max_density.tex:951: Undefined control sequence.l.951 ... \nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  )  \mright]./max_density.tex:951: Undefined control sequence.l.951 ...!\!\mathsf{G}}\mleft({U}\mright)  \mright                                                  ]

./max_density.tex:953: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.953 \end{lemma}                 

./max_density.tex:954: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.954 \begin{proof}                   ./max_density.tex:955: Undefined control sequence.l.955     Following the argument of \hyperref                                             [lemma:small:large:a]{Lemma~\re...

./max_density.tex:956: Undefined control sequence.l.956     $\nabla_{\!\!\mathsf{G}}\mleft                                        ({U}\mright) \geq \mathcalb{d}/60$, ...

./max_density.tex:956: Undefined control sequence.l.956 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \geq \mathcalb{d}/60$, w...

./max_density.tex:956: Undefined control sequence.l.956 ...thsf{G}}\mleft({U}\mright) \geq \mathcalb                                                  {d}/60$, we have that./max_density.tex:957: Undefined control sequence.l.957     ${\mathbb                   {E}}\mleft[ X \mright] = \Omega(k\cdot \psi \nabla_{\!\!\...

./max_density.tex:957: Undefined control sequence.l.957     ${\mathbb{E}}\mleft                             [ X \mright] = \Omega(k\cdot \psi \nabla_{\!\!\...

./max_density.tex:957: Undefined control sequence.l.957     ${\mathbb{E}}\mleft[ X \mright                                        ] = \Omega(k\cdot \psi \nabla_{\!\!\...

./max_density.tex:957: Undefined control sequence.l.957 ...k\cdot \psi \nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright))= \Omega(k\cd...

./max_density.tex:957: Undefined control sequence.l.957 ... \nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ))= \Omega(k\cdot \psi./max_density.tex:958: Undefined control sequence.l.958     \mathcalb                   {d}) = \Omega( k \cdot c \vartheta^{-2} \log n)$. Chernoff's

./max_density.tex:959: Undefined control sequence.l.959     inequality, \hyperref                               [theo:special:h:i:e]{Theorem~\ref*{theo:speci...

./max_density.tex:960: Undefined control sequence.l.960     $X \in (1\pm \vartheta) {\mathbb                                          {E}}\mleft[ X \mright]$ with proba...

./max_density.tex:960: Undefined control sequence.l.960 ...X \in (1\pm \vartheta) {\mathbb{E}}\mleft                                                  [ X \mright]$ with probabi...

./max_density.tex:960: Undefined control sequence.l.960 ... \vartheta) {\mathbb{E}}\mleft[ X \mright                                                  ]$ with probability at least./max_density.tex:961: Undefined control sequence.l.961     $1-2\exp( - \vartheta^2 {\mathbb                                          {E}}\mleft[ X \mright]/4) \geq 1 -...

./max_density.tex:961: Undefined control sequence.l.961 ...1-2\exp( - \vartheta^2 {\mathbb{E}}\mleft                                                  [ X \mright]/4) \geq 1 - 1...

./max_density.tex:961: Undefined control sequence.l.961 ...\vartheta^2 {\mathbb{E}}\mleft[ X \mright                                                  ]/4) \geq 1 - 1/n^{100k}$,...

./max_density.tex:963: Undefined control sequence.l.963     \hyperref                   [equation:interval]{Eq.~(\ref*{equation:interval}{)}}.

./max_density.tex:964: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.964 \end{proof}                 

./max_density.tex:966: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.966 \begin{lemma}                   ./max_density.tex:971: Undefined control sequence.l.971     $\nabla_{\!\!H}\mleft                               ({U}\mright) \geq (1-\alpha)\mathcalb{d}\mlef...

./max_density.tex:971: Undefined control sequence.l.971     $\nabla_{\!\!H}\mleft({U}\mright                                          ) \geq (1-\alpha)\mathcalb{d}\mlef...

./max_density.tex:971: Undefined control sequence.l.971 ...left({U}\mright) \geq (1-\alpha)\mathcalb                                                  {d}\mleft({H}\mright)$, we...

./max_density.tex:971: Undefined control sequence.l.971 ...mright) \geq (1-\alpha)\mathcalb{d}\mleft                                                  ({H}\mright)$, we have that./max_density.tex:971: Undefined control sequence.l.971 ...q (1-\alpha)\mathcalb{d}\mleft({H}\mright                                                  )$, we have that./max_density.tex:972: Undefined control sequence.l.972     $\nabla_{\!\!\mathsf{G}}\mleft                                        ({U}\mright) \geq (1-6\vartheta)(1-\...

./max_density.tex:972: Undefined control sequence.l.972 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \geq (1-6\vartheta)(1-\a...

./max_density.tex:972: Undefined control sequence.l.972 ...t) \geq (1-6\vartheta)(1-\alpha)\mathcalb                                                  {d}$, and this holds

./max_density.tex:974: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.974 \end{lemma}                 

./max_density.tex:975: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.975 \begin{proof}                   ./max_density.tex:976: Undefined control sequence.l.976 ...sest subset in $\mathsf{G}$. By \hyperref                                                  [lemma:small:large:b]{Lemm...



./max_density.tex:978: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.978     \begin{equation*}                           ./max_density.tex:979: Missing $ inserted.

<inserted text>                 $l.979         \nabla                    _{\!\!H}\mleft({X}\mright) \in (1\pm \vartheta)^3 \psi \...

./max_density.tex:979: Undefined control sequence.l.979         \nabla_{\!\!H}\mleft                                  ({X}\mright) \in (1\pm \vartheta)^3 \psi \...

./max_density.tex:979: Undefined control sequence.l.979         \nabla_{\!\!H}\mleft({X}\mright                                             ) \in (1\pm \vartheta)^3 \psi \...

./max_density.tex:979: Undefined control sequence.l.979 ...ht) \in (1\pm \vartheta)^3 \psi \mathcalb                                                  {d}\mleft({\mathsf{G}}\mri...

./max_density.tex:979: Undefined control sequence.l.979 ...1\pm \vartheta)^3 \psi \mathcalb{d}\mleft                                                  ({\mathsf{G}}\mright)./max_density.tex:979: Undefined control sequence.l.979 ...si \mathcalb{d}\mleft({\mathsf{G}}\mright                                                  )./max_density.tex:980: Undefined control sequence.l.980         \implies                      ./max_density.tex:981: Undefined control sequence.l.981         \mathcalb                       {d}\mleft({H}\mright) \geq  (1 - \vartheta)^3 \psi \m...

./max_density.tex:981: Undefined control sequence.l.981         \mathcalb{d}\mleft                                ({H}\mright) \geq  (1 - \vartheta)^3 \psi \m...

./max_density.tex:981: Undefined control sequence.l.981         \mathcalb{d}\mleft({H}\mright                                           ) \geq  (1 - \vartheta)^3 \psi \m...

./max_density.tex:981: Undefined control sequence.l.981 ...t) \geq  (1 - \vartheta)^3 \psi \mathcalb                                                  {d}./max_density.tex:983: Undefined control sequence.

<argument> \psi \mathcalb                           {d}l.983         \frac{\psi \mathcalb{d}}{2}                                         .

./max_density.tex:984: LaTeX Error: \begin{document} ended by \end{equation*}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.984     \end{equation*}                         ./max_density.tex:984: Missing $ inserted.

<inserted text>                 $l.984     \end{equation*}                         


Overfull \hbox (46.02353pt too wide) in paragraph at lines 969--985
\OT1/cmr/m/n/12 prob-a-bil-ity.   Let $\OML/cmm/m/it/12 X$ \OT1/cmr/m/n/12 be the dens-est sub-set in $\OT1/cmss/m/n/12 G$\OT1/cmr/m/n/12 . By [lemma:small:large:b]Lemma 5.1.1[],./max_density.tex:986: Undefined control sequence.l.986     By \hyperref                      [lemma:small:large:a]{Lemma~\ref*{lemma:small:large:a}...

./max_density.tex:987: Undefined control sequence.l.987 ...{V}$, with $\nabla_{\!\!\mathsf{G}}\mleft                                                  ({T}\mright) \leq \mathcal...

./max_density.tex:987: Undefined control sequence.l.987 ...$\nabla_{\!\!\mathsf{G}}\mleft({T}\mright                                                  ) \leq \mathcalb{d}/60$, w...

./max_density.tex:987: Undefined control sequence.l.987 ...thsf{G}}\mleft({T}\mright) \leq \mathcalb                                                  {d}/60$, we have./max_density.tex:988: Undefined control sequence.l.988     $\nabla_{\!\!H}\mleft                               ({T}\mright) < \psi \mathcalb{d} /5 < \mathca...

./max_density.tex:988: Undefined control sequence.l.988     $\nabla_{\!\!H}\mleft({T}\mright                                          ) < \psi \mathcalb{d} /5 < \mathca...

./max_density.tex:988: Undefined control sequence.l.988 ...\!\!H}\mleft({T}\mright) < \psi \mathcalb                                                  {d} /5 < \mathcalb{d}\mlef...

./max_density.tex:988: Undefined control sequence.l.988 ...right) < \psi \mathcalb{d} /5 < \mathcalb                                                  {d}\mleft({H}\mright)/2$, ...

./max_density.tex:988: Undefined control sequence.l.988 ...\psi \mathcalb{d} /5 < \mathcalb{d}\mleft                                                  ({H}\mright)/2$, and this./max_density.tex:988: Undefined control sequence.l.988 ...alb{d} /5 < \mathcalb{d}\mleft({H}\mright                                                  )/2$, and this./max_density.tex:991: Undefined control sequence.l.991     \sum_{k=2}^n \binom                             {n}{k}/n^{100k} \leq 1/n^{99}$../max_density.tex:994: Undefined control sequence.l.994     $\nabla_{\!\!\mathsf{G}}\mleft                                        ({U}\mright) > \mathcalb{d}/60$.  By...

./max_density.tex:994: Undefined control sequence.l.994 ...$\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) > \mathcalb{d}/60$.  By ...

./max_density.tex:994: Undefined control sequence.l.994 ...\mathsf{G}}\mleft({U}\mright) > \mathcalb                                                  {d}/60$.  By \hyperref[lem...

./max_density.tex:994: Undefined control sequence.l.994 ...mright) > \mathcalb{d}/60$.  By \hyperref                                                  [lemma:small:large:b]{Lemm...

./max_density.tex:996: Undefined control sequence.l.996     $\nabla_{\!\!H}\mleft                               ({U}\mright) \in (1\pm \vartheta)^3 \psi \nab...

./max_density.tex:996: Undefined control sequence.l.996     $\nabla_{\!\!H}\mleft({U}\mright                                          ) \in (1\pm \vartheta)^3 \psi \nab...

./max_density.tex:996: Undefined control sequence.l.996 ...eta)^3 \psi \nabla_{\!\!\mathsf{G}}\mleft                                                  ({U}\mright)$, which./max_density.tex:996: Undefined control sequence.l.996 ... \nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  )$, which./max_density.tex:999: Undefined control sequence.l.999         \nabla_{\!\!\mathsf{G}}\mleft                                           ({U}\mright) \in \frac{1}{(1\pm \...

./max_density.tex:999: Undefined control sequence.l.999 ... \nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  ) \in \frac{1}{(1\pm \vart...

./max_density.tex:1000: Undefined control sequence.l.1000         \nabla_{\!\!H}\mleft                                   ({U}\mright)../max_density.tex:1000: Undefined control sequence.l.1000         \nabla_{\!\!H}\mleft({U}\mright                                              ).

./max_density.tex:1003: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1003     \begin{equation*}                            ./max_density.tex:1004: Missing $ inserted.

<inserted text>                 $l.1004         \nabla                     _{\!\!\mathsf{G}}\mleft({U}\mright)./max_density.tex:1004: Undefined control sequence.l.1004         \nabla_{\!\!\mathsf{G}}\mleft                                            ({U}\mright)./max_density.tex:1004: Undefined control sequence.l.1004 ...\nabla_{\!\!\mathsf{G}}\mleft({U}\mright                                                  )./max_density.tex:1007: Undefined control sequence.l.1007         \nabla_{\!\!H}\mleft                                   ({U}\mright)./max_density.tex:1007: Undefined control sequence.l.1007         \nabla_{\!\!H}\mleft({U}\mright                                              )./max_density.tex:1009: Undefined control sequence.

<argument> (1-\alpha )\mathcalb                                 {d}\mleft ({H}\mright )l.1009 ...mleft({H}\mright)}{(1+\vartheta)^3 \psi}                                                  ./max_density.tex:1009: Undefined control sequence.

<argument> (1-\alpha )\mathcalb {d}\mleft                                           ({H}\mright )l.1009 ...mleft({H}\mright)}{(1+\vartheta)^3 \psi}                                                  ./max_density.tex:1009: Undefined control sequence.

<argument> ...ha )\mathcalb {d}\mleft ({H}\mright                                                   )l.1009 ...mleft({H}\mright)}{(1+\vartheta)^3 \psi}                                                  ./max_density.tex:1011: Undefined control sequence.

<argument> ... )(1 - \vartheta )^3 \psi \mathcalb                                                   {d}l.1011 ...\psi \mathcalb{d}}{(1+\vartheta)^3 \psi}                                                  ./max_density.tex:1013: Undefined control sequence.l.1013         (1-\alpha)(1-6\vartheta) \mathcalb                                                 {d},

./max_density.tex:1014: LaTeX Error: \begin{document} ended by \end{equation*}.



See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1014     \end{equation*}                          ./max_density.tex:1014: Missing $ inserted.

<inserted text>                 $l.1014     \end{equation*}                          

./max_density.tex:1016: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1016 \end{proof}                  

./max_density.tex:1020: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1020 \begin{lemma}                    ./max_density.tex:1034: Undefined control sequence.l.1034     $\nabla_{\!\!H}\mleft                                ({X}\mright)\geq(1-\varepsilon/6)\mathcalb{d...

./max_density.tex:1034: Undefined control sequence.l.1034     $\nabla_{\!\!H}\mleft({X}\mright                                           )\geq(1-\varepsilon/6)\mathcalb{d...

./max_density.tex:1034: Undefined control sequence.l.1034 ...X}\mright)\geq(1-\varepsilon/6)\mathcalb                                                  {d}\mleft({H}\mright)$. Then,

./max_density.tex:1034: Undefined control sequence.l.1034 ...)\geq(1-\varepsilon/6)\mathcalb{d}\mleft                                                  ({H}\mright)$. Then,./max_density.tex:1034: Undefined control sequence.l.1034 ...repsilon/6)\mathcalb{d}\mleft({H}\mright                                                  )$. Then,./max_density.tex:1035: Undefined control sequence.l.1035     ${\nabla}\mleft                          ({X}\mright) \geq (1-\varepsilon)\mathcalb{d}\mlef...

./max_density.tex:1035: Undefined control sequence.l.1035     ${\nabla}\mleft({X}\mright                                     ) \geq (1-\varepsilon)\mathcalb{d}\mlef...

./max_density.tex:1035: Undefined control sequence.l.1035 ...X}\mright) \geq (1-\varepsilon)\mathcalb                                                  {d}\mleft({\mathsf{G}}\mri...

./max_density.tex:1035: Undefined control sequence.l.1035 ...) \geq (1-\varepsilon)\mathcalb{d}\mleft                                                  ({\mathsf{G}}\mright)$../max_density.tex:1035: Undefined control sequence.l.1035 ...n)\mathcalb{d}\mleft({\mathsf{G}}\mright                                                  )$.

./max_density.tex:1036: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1036 \end{lemma}                  

./max_density.tex:1037: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1037 \begin{proof}                    ./max_density.tex:1039: Undefined control sequence.l.1039     and using \hyperref                              [lemma:happy]{Lemma~\ref*{lemma:happy}}.

./max_density.tex:1040: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1040 \end{proof}                  [13]

./max_density.tex:1050: LaTeX Error: Environment compactenumI undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1050 \begin{compactenumI}                           [itemsep=-0.5ex]

./max_density.tex:1051: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1051     \item B                  uild the data-structure of \hyperref[cor:disks-estimate]{C...

./max_density.tex:1051: Undefined control sequence.l.1051 ...em Build the data-structure of \hyperref                                                  [cor:disks-estimate]{Corol...




LaTeX Warning: Citation `l-nopkn-22' on page 14 undefined on input line 1054.



./max_density.tex:1056: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1056     \item F                  or each object $\mathsf{o} \in \mathcal{D}$, query the dat...

./max_density.tex:1057: Undefined control sequence.l.1057     of \hyperref                       [cor:disks-estimate]{Corollary~\ref*{cor:disks-estima...




Overfull \hbox (36.06775pt too wide) in paragraph at lines 1056--1063
[]\OT1/cmr/m/n/12 For each ob-ject $\OT1/cmss/m/n/12 o \OMS/cmsy/m/n/12 2 D$\OT1/cmr/m/n/12 , query the data-structure of [cor:disks-estimate]Corollary 3.2.3[]

./max_density.tex:1064: LaTeX Error: Lonely \item--perhaps a missing list environment.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1064     \item W                  e perform $|F|$ iterations and in each iteration,./max_density.tex:1070: Undefined control sequence.l.1070     data-structure of \hyperref                                      [cor:disks-estimate]{Corollary~\ref*{c...



./max_density.tex:1073: LaTeX Error: \begin{document} ended by \end{compactenumI}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1073 \end{compactenumI}                         

./max_density.tex:1077: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1077 \begin{lemma}                    %

./max_density.tex:1083: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1083 \end{lemma}                  

./max_density.tex:1084: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1084 \begin{proof}                    

./max_density.tex:1090: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1090     \begin{equation*}                            ./max_density.tex:1091: Missing $ inserted.

<inserted text>                 $l.1091         {d} \geq                        \frac{1}{\varepsilon}\cdot\frac{1+ \varepsilon/c}{1/...



./max_density.tex:1092: LaTeX Error: \begin{document} ended by \end{equation*}.



See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1092     \end{equation*}                          ./max_density.tex:1092: Missing $ inserted.

<inserted text>                 $l.1092     \end{equation*}                          

./max_density.tex:1098: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1098     \begin{equation*}                            ./max_density.tex:1099: Missing $ inserted.

<inserted text>                 $l.1099         d_                 {\mathsf{o}}=d' \in (1\pm \varepsilon/c''){d}.

./max_density.tex:1100: LaTeX Error: \begin{document} ended by \end{equation*}.



See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1100     \end{equation*}                          ./max_density.tex:1100: Missing $ inserted.

<inserted text>                 $l.1100     \end{equation*}                          

./max_density.tex:1101: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1101 \end{proof}                  

./max_density.tex:1103: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1103 \begin{lemma}                    [14]

./max_density.tex:1106: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1106 \end{lemma}                  

./max_density.tex:1107: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1107 \begin{proof}                    

./max_density.tex:1118: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1118     \begin{equation*}                            ./max_density.tex:1119: Missing $ inserted.

<inserted text>                 $l.1119 ...rac{d_{\mathsf{o}}}{\sum d_{\mathsf{o}}}                                                  \cdot \underbrace{\frac{1\...

./max_density.tex:1119: Missing $ inserted.

<inserted text>                 $l.1119 ...rac{d_{\mathsf{o}}}{\sum d_{\mathsf{o}}}                                                  \cdot \underbrace{\frac{1\...

./max_density.tex:1119: Missing $ inserted.

<inserted text>                 $l.1119 ...rac{d_{\mathsf{o}}}{\sum d_{\mathsf{o}}}                                                  \cdot \underbrace{\frac{1\...

./max_density.tex:1119: Extra }, or forgotten $.\frac  #1#2->{\begingroup #1\endgroup \over #2}                                               l.1119 ...rac{d_{\mathsf{o}}}{\sum d_{\mathsf{o}}}                                                  \cdot \underbrace{\frac{1\...

./max_density.tex:1119: Undefined control sequence.l.1119 ...race{\frac{1\pm\varepsilon/c}{d}}_{\text                                                  {almost-uniformity}} \subs...

./max_density.tex:1120: Undefined control sequence.

<argument> ...\pm \varepsilon /c'')2m}_{\hyperref                                                   [lemma:approx-degree]{Lemm...l.1120 ...ree]{Lemma~\ref*{lemma:approx-degree}}}}                                                  \cdot

./max_density.tex:1125: LaTeX Error: \begin{document} ended by \end{equation*}.



See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1125     \end{equation*}                          ./max_density.tex:1125: Missing $ inserted.

<inserted text>                 $l.1125     \end{equation*}                          ./max_density.tex:1125: Missing } inserted.

<inserted text>                 }l.1125     \end{equation*}                          


Overfull \hbox (134.29846pt too wide) in paragraph at lines 1113--1126
\OT1/cmr/m/n/12 prob-a-bil-ity lower-bounded by:  d$[]$$[]$ 

./max_density.tex:1130: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1130 \end{proof}                  

./max_density.tex:1132: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1132 \begin{lemma}                    

./max_density.tex:1135: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1135 \end{lemma}                  

./max_density.tex:1136: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1136 \begin{proof}                    ./max_density.tex:1141: Undefined control sequence.l.1141     data-structure of \hyperref                                      [cor:disks-estimate]{Corollary~\ref*{c...



./max_density.tex:1145: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1145 \end{proof}                  

./max_density.tex:1149: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1149 \begin{lemma}                    

./max_density.tex:1162: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1162 \end{lemma}                  

./max_density.tex:1166: LaTeX Error: Environment theorem undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1166 \begin{theorem}                      

./max_density.tex:1175: LaTeX Error: \begin{document} ended by \end{theorem}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1175 \end{theorem}                    

./max_density.tex:1176: LaTeX Error: Environment proof undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1176 \begin{proof}                    ./max_density.tex:1179: Undefined control sequence.l.1179 ...n\log n)$ expected time (using \hyperref                                                  [lemma:sweepline]{Lemma~\r...




Overfull \hbox (6.59183pt too wide) in paragraph at lines 1169--1180
\OT1/cmr/m/n/12 be han-dled di-rectly by com-put-ing the whole in-ter-sec-tion graph in $\OML/cmm/m/it/12 O\OT1/cmr/m/n/12 (\OML/cmm/m/it/12 "[]n [] n\OT1/cmr/m/n/12 )$./max_density.tex:1181: Undefined control sequence.l.1181 ... handle the other case, we use \hyperref                                                  [lemma:random-sampler]{Lem...

./max_density.tex:1185: Undefined control sequence.l.1185     edges, using \hyperref                                 [lemma:sampling]{Lemma~\ref*{lemma:sampling...




LaTeX Warning: Citation `bgm-epgam-14' on page 15 undefined on input line 1187.





./max_density.tex:1189: LaTeX Error: \begin{document} ended by \end{proof}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1189 \end{proof}                  [15]


LaTeX Warning: Citation `ah-adrp-08' on page 16 undefined on input line 1201.

./max_density.tex:1212: Undefined control sequence.l.1212 \printbibliography                         


LaTeX Warning: Citation `mr-ra-95' on page 16 undefined on input line 1219.



./max_density.tex:1221: LaTeX Error: Environment lemma undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1221 \begin{lemma}                    ./max_density.tex:1226: Undefined control sequence.l.1226         {\mathbb                       {P}}\mleft[  X_i = 1  \mright] =p_i,./max_density.tex:1226: Undefined control sequence.l.1226         {\mathbb{P}}\mleft                                 [  X_i = 1  \mright] =p_i,./max_density.tex:1226: Undefined control sequence.l.1226 ...   {\mathbb{P}}\mleft[  X_i = 1  \mright                                                  ] =p_i,./max_density.tex:1230: Undefined control sequence.l.1230         {\mathbb                       {P}}\mleft[  X_i = 0  \mright] =1- p_i,./max_density.tex:1230: Undefined control sequence.l.1230         {\mathbb{P}}\mleft                                 [  X_i = 0  \mright] =1- p_i,./max_density.tex:1230: Undefined control sequence.l.1230 ...   {\mathbb{P}}\mleft[  X_i = 0  \mright                                                  ] =1- p_i,./max_density.tex:1233: Undefined control sequence.l.1233     $\mu = {\mathbb                          {E}}\mleft[ \bigl. X \mright] = \sum_i p_i$.  For ...

./max_density.tex:1233: Undefined control sequence.l.1233     $\mu = {\mathbb{E}}\mleft                                    [ \bigl. X \mright] = \sum_i p_i$.  For ...

./max_density.tex:1233: Undefined control sequence.l.1233 ...u = {\mathbb{E}}\mleft[ \bigl. X \mright                                                  ] = \sum_i p_i$.  For $\de...

./max_density.tex:1234: Undefined control sequence.l.1234     ${\mathbb                    {P}}\mleft[  \bigl. X > (1+\delta)\mu  \mright] < 2^{-\m...

./max_density.tex:1234: Undefined control sequence.l.1234     ${\mathbb{P}}\mleft                              [  \bigl. X > (1+\delta)\mu  \mright] < 2^{-\m...

./max_density.tex:1234: Undefined control sequence.l.1234 ...left[  \bigl. X > (1+\delta)\mu  \mright                                                  ] < 2^{-\mu (1 + \delta)}$.

./max_density.tex:1235: LaTeX Error: \begin{document} ended by \end{lemma}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1235 \end{lemma}                  

./max_density.tex:1237: LaTeX Error: Environment theorem undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1237 \begin{theorem}                      ./max_density.tex:1242: Undefined control sequence.l.1242 ...um_{i=1}^n X_i$, and let $\mu = {\mathbb                                                  {E}}\mleft[ X \mright]$. W...

./max_density.tex:1242: Undefined control sequence.l.1242 ... X_i$, and let $\mu = {\mathbb{E}}\mleft                                                  [ X \mright]$. We have that./max_density.tex:1242: Undefined control sequence.l.1242 ...let $\mu = {\mathbb{E}}\mleft[ X \mright                                                  ]$. We have that

./max_density.tex:1243: LaTeX Error: Environment equation* undefined.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1243     \begin{equation*}                            ./max_density.tex:1244: Missing $ inserted.

<inserted text>                 $l.1244         \displaystyle                            %./max_density.tex:1245: Undefined control sequence.l.1245         {\mathbb                       {P}}\mleft[ \bigl.{X} \notin (1\pm \varepsilon) \mu  ...

./max_density.tex:1245: Undefined control sequence.l.1245         {\mathbb{P}}\mleft                                 [ \bigl.{X} \notin (1\pm \varepsilon) \mu  ...

./max_density.tex:1245: Undefined control sequence.l.1245 ...} \notin (1\pm \varepsilon) \mu  \mright                                                  ]%./max_density.tex:1247: Undefined control sequence.l.1247         2 \exp\mleft                           ({ -\varepsilon^2 \mu / 3}\mright)./max_density.tex:1247: Undefined control sequence.l.1247 ...p\mleft({ -\varepsilon^2 \mu / 3}\mright                                                  )

./max_density.tex:1248: LaTeX Error: \begin{document} ended by \end{equation*}.



See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1248     \end{equation*}                          ./max_density.tex:1248: Missing $ inserted.

<inserted text>                 $l.1248     \end{equation*}                          

./max_density.tex:1249: LaTeX Error: \begin{document} ended by \end{theorem}.

See the LaTeX manual or LaTeX Companion for explanation.Type  H <return>  for immediate help. ...                                                                                                l.1249 \end{theorem}                    [16] (junk/max_density.aux)


LaTeX Warning: There were undefined references.




LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )

(see the transcript file for additional information)</usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr17.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr8.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmss10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmss12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmss8.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy8.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmti10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmti12.pfb></usr/share/texmf/fonts/type1/public/cm-super/sfrm0700.pfb></usr/share/texmf/fonts/type1/public/cm-super/sfrm1000.pfb>

Output written on junk/max_density.pdf (16 pages, 336776 bytes).SyncTeX written on junk/max_density.synctex.gz.
Transcript written on junk/max_density.log.
